Expressibility in the Lambda Calculus with mu

We address a problem connected to the unfolding semantics of functional programming languages: give a useful characterization of those infinite lambda-terms that are lambda_{letrec}-expressible in the sense that they arise as infinite unfoldings of terms in lambda_{letrec}, the lambda-calculus with letrec. We provide two characterizations, using concepts we introduce for infinite lambda-terms: regularity, strong regularity, and binding-capturing chains. It turns out that lambda_{letrec}-expressible infinite lambda-terms form a proper subclass of the regular infinite lambda-terms. In this paper we establish these characterizations only for expressibility in lambda_{mu}, the lambda-calculus with explicit mu-recursion. We show that for all infinite lambda-terms T the following are equivalent: (i): T is lambda_{mu}-expressible; (ii): T is strongly regular; (iii): T is regular, and it only has finite binding-capturing chains. We define regularity and strong regularity for infinite lambda-terms as two different generalizations of regularity for infinite first-order terms: as the existence of only finitely many subterms that are defined as the reducts of two rewrite relations for decomposing lambda-terms. These rewrite relations act on infinite lambda-terms furnished with a marked prefix of abstractions for collecting decomposed lambda-abstractions and keeping the terms closed under decomposition. They differ in how vacuous abstractions in the prefix are removed. This report accompanies the article with the same title for the proceedings of the conference RTA 2013, and mainly differs from that by providing the proof of the characterization of lambda_{mu}-expressibility with binding-capturing chains.

==> figs/pstricks/Makefile <==
# create a picture for each file containing a Lagtx fragment in the directory

# disable implicit rules
.SUFFIXES:

TEXFILES=$(wildcard *.tex)

#noflags:
#	make -r default

default: pdfs
	make -C ltgs

epss: $(TEXFILES:.tex=.lgr.eps)
pdfs: $(TEXFILES:.tex=.lgr.pdf)

%.lgr.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/lambdagraph}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

include mk/figure.mk


==> figs/pstricks/entangled.tex <==
\lambdaterm{\abs{x}{\abs{y}{\app
		{\abs{x}{\app
			{\abs{y}{\app
				{\etc}
				{\s{\var x}}
			}}
			{\s{\var y}}
		}}
		{\s{\var x}}
}}}


==> figs/pstricks/ltgs/Makefile <==
# create a picture for each file containing a Lagtx fragment in the directory

# disable implicit rules
.SUFFIXES:

TEXFILES=$(wildcard *.tex)

#noflags:
#	make -r default

default: pdfs

epss: $(TEXFILES:.tex=.ltg.eps)
pdfs: $(TEXFILES:.tex=.ltg.pdf)

%.ltg.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/ltg}' >> $@
	echo '\\newcommand\\nlabel[1]{#1}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

include mk/figure.mk


==> figs/pstricks/ltgs/entangled.tex <==
\lambdaterm{
\abs{() U}{
\abs{(\lambda x)~ R(x)}{
\app{(\lambda xy)~R(y)~x}{
\del{(\lambda xy)~R(y)}{
\abs{(\lambda y)~R(y)}{
\etc}}}{
\del{(\lambda xy)~x}{
\var{(\lambda x)~x}}}}}}


==> figs/pstricks/ltgs/macros/lambdagraph.tex <==
% Named Lambda Graph with Invisible Scopes

\newcommand\tree[2]{\pstree[linewidth=0.5pt,nodesep=0.4mm,levelsep=0.8cm]{#1}{#2}}
\newcommand\node[1]{\TR{#1}}

% The Language

\newcommand\lambdaterm[1]{\ensuremath{\tree{\nil}{#1}}}

\newcommand\letbind[2]{\rnode[t]{#1}{#2}}
% with explicit sharing node
%\newcommand\letbind[2]{\tree{\node{\rnode[t]{#1}{\vphantom{i}\pstriangle(0mm,3.28mm)(6mm,-3.9mm)}}}{#2}}
\newcommand\letvar[1]{{\psset{nodesepB=0pt}\Tp*[name=here]}\ncangles[nodesepA=0pt,angleB=70]{-}{here}{#1}}
\newcommand\letvara[3]{{\psset{nodesepB=0pt}\Tp*[name=here]}\ncangles[nodesepA=0pt,angleA=#2,angleB=#3]{-}{here}{#1}}
\newcommand\abs[2]{\tree{\node{\lambda #1}}{#2}}
\newcommand\s[1]{#1}
\newcommand\sA[1]{#1}
\newcommand\cpr[2]{#2}
\newcommand\cpR[2]{#2}
\newcommand\app[2]{\tree{\node{@}}{#1 #2}}
\newcommand\var[1]{\node{#1}}
\newcommand\vara[3]{\node{#1}}

\newcommand\sapp[3]{\app{#2}{#3}}
\newcommand\cprapp[4]{\app{#3}{#4}}

\newcommand\etc[0]{\node{\vdots}}
\newcommand\op[1]{\Tcircle{#1}}
\newcommand\nil{\node{}}


==> figs/pstricks/ltgs/macros/ltg.tex <==
% The Lambda Transition Graph

\newcommand\node[1]{\TR{#1}}
\newcommand\putEdge[1]{\mput*{#1}}
\newcommand\tree[2]{\pstree[arrows=->,treesep=4mm,levelsep=1.3cm]{#1}{#2}}
%\newcommand\lambdaterm[1]{\ensuremath{\tree{\nil{}}{#1{ }}}}
\newcommand\lambdaterm[1]{\ensuremath{#1{}}}
\newcommand\nil[1]{\node{}\putEdge{#1}}
\newcommand\etc[1]{\node{\vdots}\putEdge{#1}}

\newcommand\abs[3]{\tree{\node{#1}\putEdge{#3}}{#2{\lambda}}}
\newcommand\app[4]{\tree{\node{#1}\putEdge{#4}}{#2{@_0} #3{@_1}}}
\newcommand\s[3]{\tree{\node{#1}\putEdge{#3}}{#2{S}}}
\newcommand\del[3]{\tree{\node{#1}\putEdge{#3}}{#2{del}}}
\newcommand\var[2]{\node{#1{}}\putEdge{#2}}


==> figs/pstricks/ltgs/mk/postlude.tex <==
\end{document}


==> figs/pstricks/ltgs/simpleletrec.tex <==
\lambdaterm{
\abs{() T}{
\abs{(\lambda x)~\lambda y. T\,y~x}{
\app{(\lambda xy)~T\,y~x}
{
\app{(\lambda xy)~T\,y}
{
\s{(\lambda xy)~T}{
\s{(\lambda x)~T}{
\var{()~T}
}
}}
{
\var{(\lambda xy)~y}
}
}
{
\s{(\lambda xy)~x}
{\var{(\lambda x)~x}}
}
}}}


==> figs/pstricks/macros/lambdagraph.tex <==
% Named Lambda Graph with Invisible Scopes

\newcommand\tree[2]{\pstree[linewidth=0.5pt,nodesep=0.4mm,levelsep=0.8cm]{#1}{#2}}
\newcommand\node[1]{\TR{#1}}

% The Language

\newcommand\lambdaterm[1]{\ensuremath{\tree{\nil}{#1}}}

\newcommand\letbind[2]{\rnode[t]{#1}{#2}}
% with explicit sharing node
%\newcommand\letbind[2]{\tree{\node{\rnode[t]{#1}{\vphantom{i}\pstriangle(0mm,3.28mm)(6mm,-3.9mm)}}}{#2}}
\newcommand\letvar[1]{{\psset{nodesepB=0pt}\Tp*[name=here]}\ncangles[nodesepA=0pt,angleB=70]{-}{here}{#1}}
\newcommand\letvara[3]{{\psset{nodesepB=0pt}\Tp*[name=here]}\ncangles[nodesepA=0pt,angleA=#2,angleB=#3]{-}{here}{#1}}
\newcommand\abs[2]{\tree{\node{\lambda #1}}{#2}}
\newcommand\s[1]{#1}
\newcommand\sA[1]{#1}
\newcommand\cpr[2]{#2}
\newcommand\cpR[2]{#2}
\newcommand\app[2]{\tree{\node{@}}{#1 #2}}
\newcommand\var[1]{\node{#1}}
\newcommand\vara[3]{\node{#1}}

\newcommand\sapp[3]{\app{#2}{#3}}
\newcommand\cprapp[4]{\app{#3}{#4}}

\newcommand\etc[0]{\node{\vdots}}
\newcommand\op[1]{\Tcircle{#1}}
\newcommand\nil{\node{}}


==> figs/pstricks/macros/ltg-bl.tex <==
% Lambda Transition Graph with Back-Links

% CAUTION: The lambda-letrec constructors are supposed to be used as unsaturated functions.
%          The last two parameters are all supplied here.
%          First paramater: labelling of the incoming edge
%          Second paramater: labelling of this node

\newcommand\mkNode\Toval
\newcommand\putEdge{\mput*}
\newcommand\tree[2]{\pstree[arrows=->,treesep=1cm,levelsep=1.5cm]{#1}{#2}}
\newcommand\node[1]{\mkNode{\nlabel{#1}}}


% The Language

%\newcommand\lambdaterm[1]{\ensuremath{\tree{\TR{}}{#1{}{}}}}
\newcommand\lambdaterm[1]{\ensuremath{#1{}{}}}

\newcommand\app[4]{\tree{\node{#4}#3}{#1{\putEdge{@_0}}{#4} #2{\putEdge{@_1}}{#4}}}

\newcommand\abs[4]{\tree{\rnode{#1}{\node{#4}}#3}{#2{\putEdge\lambda}{#4#1}}}

\newcommand\s[3]{
	\StrGobbleRight{#3}1[\NewStr]
	\tree{\node{#3}#2}{#1{\putEdge S}\NewStr}
}

\newcommand\sA[3]{
	\StrGobbleRight{#3}1[\NewStri]
	\tree{\node{#3}#2}{#1{\putEdge S}\NewStri}
}

\newcommand\sapp[5]{
	\StrGobbleRight{#5}1[\NewStri]
	\tree{\node{#5}#4}{#1{\putEdge S}\NewStri #2{\putEdge{@_0}}{#5} #3{\putEdge{@_1}}{#5}}
}

\newcommand\cprapp[6]{
	\StrDel[1]{#6}{#1}[\ANewStrin]
	\tree{\node{#6}#5}{#2{\putEdge{del}}\ANewStrin #3{\putEdge{@_0}}{#6} #4{\putEdge{@_1}}{#6}}
}

\newcommand\cpr[4]{
	\StrDel[1]{#4}{#1}[\NewStrin]
	\tree{\node{#4}#3}{#2{\putEdge{del}}\NewStrin}
}

\newcommand\cpR[4]{
	\StrDel[1]{#4}{#1}[\NewString]
	\tree{\node{#4}#3}{#2{\putEdge{del}}\NewString}
}

\newcommand\var[3]{{\psset{nodesepB=0pt}\mkNode[name=here]{\nlabel{#3}}#2}\ncangles[nodesepA=0pt]{->}{here}{#1}\ncput*{0}}
\newcommand\vara[5]{{\psset{nodesepB=0pt}\mkNode[name=here]{\nlabel{#5}}#4}\ncangles[nodesepA=0pt,angleA=#2,angleB=#3]{->}{here}{#1}\ncput*{0}}

\newcommand\etc[2]{\TR{\vdots}#1}

\newcommand\letbind[4]{#2{\rnode{#1}{}#3}{#4}}

\newcommand\letvar[3]{{\psset{arrows=-,nodesepB=0pt}\Tp*[name=here]}\ncangles[angleB=70,nodesepA=0pt]{->}{here}{#1}#2}
\newcommand\letvara[5]{{\psset{arrows=-,nodesepB=0pt}\Tp*[name=here]}\ncangles[angleA=#2,angleB=#3,nodesepA=0pt]{->}{here}{#1}#4}

%\newcommand\op[3]{\tree{\node{#3}#2}{\mkNode{#1}}}
%\newcommand\op[3]{\var{#1}{#2}{#3}}
%\newcommand\op[3]{\etc{#2}{#3}}
\newcommand\op[3]{\TR{\dots}#2}

\newcommand\nil[2]{\node{#2}#1}


==> figs/pstricks/macros/ltg.tex <==
% The Lambda Transition Graph

\input{macros/lambdagraph}

\renewcommand\abs[2]{\tree{\node{#1}}{#2{\putEdge\lambda}}}
\renewcommand\s[2]{\tree{\node{#1}}{#2{\putEdge S}}}
\renewcommand\del[2]{\tree{\node{#1}}{#2{\putEdge{del}}}}
\renewcommand\var[1]{\node{#1}}


==> figs/pstricks/macros/scopedgraph.tex <==
% Nameless Lambda Graph with Visible Scopes

\input{macros/lambdagraph}

\renewcommand\abs[2]{\tree{\node{\lambda}}{#2}}
\renewcommand\s[1]{\tree{\node S}{#1}}
\renewcommand\del[1]{\tree{\node{del}}{#1}}
\renewcommand\var[1]{\node{0}}
\renewcommand\vara[3]{\node{0}}


==> figs/pstricks/mk/postlude.tex <==
\end{document}


==> figs/pstricks/simpleletrec-unf.tex <==
% λx.letrec f = λy.f yx in f ]

\lambdaterm{\abs{x}{\abs{y}{\app{\app{\abs{x}{\abs{y}{\app{\app\etc{\var y}}{\s{\var x}}}}}{\var y}}{\s{\var x}}}}}

